How Useful is Intermittent, Asynchronous Expert Feedback for Bayesian Optimization?

Bayesian optimization (BO) is an integral part of automated scientific discovery -- the so-called self-driving lab -- where human inputs are ideally minimal or at least non-blocking. However, scientists often have strong intuition, and thus human feedback is still useful. Nevertheless, prior works in enhancing BO with expert feedback, such as by incorporating it in an offline or online but blocking (arrives at each BO iteration) manner, are incompatible with the spirit of self-driving labs. In this work, we study whether a small amount of randomly arriving expert feedback that is being incorporated in a non-blocking manner can improve a BO campaign. To this end, we run an additional, independent computing thread on top of the BO loop to handle the feedback-gathering process. The gathered feedback is used to learn a Bayesian preference model that can readily be incorporated into the BO thread, to steer its exploration-exploitation process. Experiments on toy and chemistry datasets suggest that even just a few intermittent, asynchronous expert feedback can be useful for improving or constraining BO. This can especially be useful for its implication in improving self-driving labs, e.g. making them more data-efficient and less costly.

==> contents_aabi/03_method.tex <==
%!TEX root = ../main_aabi.tex

\section{Asynchronously Incorporating Expert Intuition in BO}
\label{sec:method_bo}

We present the three integral components for asynchronously incorporating expert intuition on top of a standard BO.
They are: (i) a surrogate model for the expert feedback (\cref{subsec:surrogate_pref}), (ii) an acquisition function to combine the said feedback into a BO loop (\cref{subsec:thompson_sampling_pref}), and finally, (iii) an active learning mechanism to present the most informative pairwise comparisons to the expert (\cref{subsec:active_learning_pref}).
The overall system is summarized in \cref{fig:algo}. \Sriram{I haven't seen it so far, but we should have a paragraph dedicated to what is new in our work and why this is helpful. We can have it either here or somewhere earlier.}


\subsection{Surrogate model for expert intuition}
\label{subsec:surrogate_pref}

Let \(\argmax_{x \in \X} f(x)\) be a BO problem, maximizing a black-box \(f: \X \to \Y\).
For instance, consider the problem of finding a better material for a battery: \(x\) is a candidate molecule to be used to make the battery, and \(f(x)\) is the energy density of the said battery.
In addition to performing the above maximization, our other goal is to model expert intuition about which molecules are preferable, e.g.\ in terms of costs, synthesizability, regulations, etc.
\gp{We haven't mentioned at all how we use expert intuition/perferences. Right now we just talk about collecting it, but how it's used is still a mystery to the reader.}

We propose to capture this latent expert intuition by maintaining a LLA-approximated Bayesian belief \(p(r \mid \Dpref)\) under the Bradley-Terry NN model \(r_\psi: \X \to \R\) \eqref{eq:bradley_terry_lik} and \(\Dpref = \{x_{i0}, x_{i1}, \ell_i\}_{i=1}^m\).
Note that, just like the marginal belief of the standard BO \(p(f(x) \mid x, \D)\), the marginal belief \(p(r(x) \mid x, \Dpref)\) about an expert intuition is also a Gaussian.


\subsection{Acquisition function for combining expert intuition}
\label{subsec:thompson_sampling_pref}

\ak{
    \begin{itemize}
        \item Difference human feedback types
        \item Different methodology for different type of human feedback
    \end{itemize}
}

While our formulation deviates from the standard multiobjective BO, we can still take inspiration on how to incorporate the reward model \(r\) into the mix when optimizing \(f\) via the BO surrogate \(p(f \mid \D)\).
Consider the Thompson sampling acquisition function.
One can simply augment it with the \(r\) via:
%
\begin{equation} \label{eq:expats}
  \expat(x; \gamma) := \hat{f}(x) + \gamma \hat{r}(x) \qquad \text{with} \enspace \hat{f} \sim p(f \mid \D) \enspace \text{and} \enspace \hat{r} \sim p(r \mid \Dpref) ,
\end{equation}
%
where \(\gamma \geq 0\) controls how much do we want to believe the expert's intuition.
We call this acquisition function \defword{Expert-Preference Aware Thompson Sampling (ExpaTS)}.
\gp{After all the talk about using expert intuition and preferences, we then simply say we're using a linearization and don't justify why this is the proper way to incorporate expert feedback. A much more detailed justification would also help clarify the ``intuition-versus-preferences'' vagueness throughout the paper.}

That is, \(\expat\) can be seen as a multiobjective Thompson sampling with linear scalarization \citep{paria2020flexible} over the two objectives: maximizing \(f\) and maximizing an abstract expert intuition.
Unlike standard multiobjective BO, however, this acquisition function is non-destructive to the original problem since the second objective is optional and decoupled from the original BO problem, and moreover \(\expat\) reverts back to the standard Thompson sampling by setting \(\gamma = 0\).
Nevertheless, when \(\gamma > 0\), both \(\hat{f}\) and \(\hat{r}\) are optimized jointly, e.g.\ via SGD when \(\X\) is a continuous space.


\subsection{Expert feedback selection}
\label{subsec:active_learning_pref}

It is important to make expert-preference learning as data-efficient as possible.
This is because, first, the spirit of SDL is to minimize human interference, and second, data annotation is a tedious process and the expert might be much more useful elsewhere.
The proposed framework is compatible with any top-\(k\) selection criteria in the expert feedback thread; the simplest being a random selection strategy.
Let \(\D_\text{cand} := \{(x_{i0}, x_{i1})\}_{i=1}^{m}\) be pairs generated from the current observations \(\D_t\).
We can then simply obtain \(\{\beta(x_{i0}, x_{i1})\}_{i=1}^m\) and pick \(k\) pairs uniformly at random.
\gp{Given that we have a probabilistic model of preferences, why are we not using a probabilistic acquisition function here? I imagine this non-Bayesian criterion will be especially controversial at AABI :)}
These pairs are then presented to an expert, and the expert can choose to annotate (some of) them.
Alternatively, other more sophisticated active learning acquisition functions such as BALD \citep{houlsby2011bald} can be employed.

